Vaex: Big Data exploration in the era of Gaia

We present a new Python library called vaex, to handle extremely large tabular datasets, such as astronomical catalogues like the Gaia catalogue, N-body simulations or any other regular datasets which can be structured in rows and columns. Fast computations of statistics on regular N-dimensional grids allows analysis and visualization in the order of a billion rows per second. We use streaming algorithms, memory mapped files and a zero memory copy policy to allow exploration of datasets larger than memory, e.g. out-of-core algorithms. Vaex allows arbitrary (mathematical) transformations using normal Python expressions and (a subset of) numpy functions which are lazily evaluated and computed when needed in small chunks, which avoids wasting of RAM. Boolean expressions (which are also lazily evaluated) can be used to explore subsets of the data, which we call selections. Vaex uses a similar DataFrame API as Pandas, a very popular library, which helps migration from Pandas. Visualization is one of the key points of vaex, and is done using binned statistics in 1d (e.g. histogram), in 2d (e.g. 2d histograms with colormapping) and 3d (using volume rendering). Vaex is split in in several packages: vaex-core for the computational part, vaex-viz for visualization mostly based on matplotlib, vaex-jupyter for visualization in the Jupyter notebook/lab based in IPyWidgets, vaex-server for the (optional) client-server communication, vaex-ui for the Qt based interface, vaex-hdf5 for hdf5 based memory mapped storage, vaex-astro for astronomy related selections, transformations and memory mapped (column based) fits storage. Vaex is open source and available under MIT license on github, documentation and other information can be found on the main website: https://vaex.io, https://docs.vaex.io or https://github.com/maartenbreddels/vaex

==> aas_macros.tex <==
%
%  These Macros are taken from the AAS TeX macro package version 4.0.
%  Include this file in your LaTeX source only if you are not using
%  the AAS TeX macro package and need to resolve the macro definitions
%  in the BibTeX entries returned by the ADS abstract service.
%
%  If you plan not to use this file to resolve the journal macros
%  rather than the whole AAS TeX macro package, you should save the
%  file as ``aas_macros.sty'' and then include it in your paper by
%  using a construct such as:
%	\documentstyle[11pt,aas_macros]{article}
%
%  For more information on the AASTeX macro package, please see the URL
%	http://www.aas.org/publications/aastex.html
%  For more information about ADS abstract server, please see the URL
%	http://adswww.harvard.edu/ads_abstracts.html
%

% Abbreviations for journals.  The object here is to provide authors
% with convenient shorthands for the most "popular" (often-cited)
% journals; the author can use these markup tags without being concerned
% about the exact form of the journal abbreviation, or its formatting.
% It is up to the keeper of the macros to make sure the macros expand
% to the proper text.  If macro package writers agree to all use the
% same TeX command name, authors only have to remember one thing, and
% the style file will take care of editorial preferences.  This also
% applies when a single journal decides to revamp its abbreviating
% scheme, as happened with the ApJ (Abt 1991).
\newcommand\aj{{AJ}}                   % Astronomical Journal
\newcommand\araa{{ARA\&A}}             % Annual Review of Astron and Astrophys
\newcommand\apj{{ApJ}}                 % Astrophysical Journal
\newcommand\apjl{{ApJ}}                % Astrophysical Journal, Letters
\newcommand\apjs{{ApJS}}               % Astrophysical Journal, Supplement
\newcommand\ao{{Appl.~Opt.}}           % Applied Optics
\newcommand\apss{{Ap\&SS}}             % Astrophysics and Space Science
\newcommand\aap{{A\&A}}                % Astronomy and Astrophysics
\newcommand\aapr{{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\newcommand\aaps{{A\&AS}}              % Astronomy and Astrophysics, Supplement
\newcommand\azh{{AZh}}                 % Astronomicheskii Zhurnal
\newcommand\baas{{BAAS}}               % Bulletin of the AAS
\newcommand\jrasc{{JRASC}}             % Journal of the RAS of Canada
\newcommand\memras{{MmRAS}}            % Memoirs of the RAS
\newcommand\mnras{{MNRAS}}             % Monthly Notices of the RAS
\newcommand\pra{{Phys.~Rev.~A}}        % Physical Review A: General Physics
\newcommand\prb{{Phys.~Rev.~B}}        % Physical Review B: Solid State
\newcommand\prc{{Phys.~Rev.~C}}        % Physical Review C
\newcommand\prd{{Phys.~Rev.~D}}        % Physical Review D
\newcommand\pre{{Phys.~Rev.~E}}        % Physical Review E
\newcommand\prl{{Phys.~Rev.~Lett.}}    % Physical Review Letters
\newcommand\pasp{{PASP}}               % Publications of the ASP
\newcommand\pasj{{PASJ}}               % Publications of the ASJ
\newcommand\qjras{{QJRAS}}             % Quarterly Journal of the RAS
\newcommand\skytel{{S\&T}}             % Sky and Telescope
\newcommand\solphys{{Sol.~Phys.}}      % Solar Physics
\newcommand\sovast{{Soviet~Ast.}}      % Soviet Astronomy
\newcommand\ssr{{Space~Sci.~Rev.}}     % Space Science Reviews
\newcommand\zap{{ZAp}}                 % Zeitschrift fuer Astrophysik
\newcommand\nat{{Nature}}              % Nature
\newcommand\iaucirc{{IAU~Circ.}}       % IAU Cirulars
\newcommand\aplett{{Astrophys.~Lett.}} % Astrophysics Letters
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\newcommand\grl{{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\newcommand\jcp{{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\newcommand\jgr{{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\newcommand\nphysa{{Nucl.~Phys.~A}}   % Nuclear Physics A
\newcommand\physrep{{Phys.~Rep.}}   % Physics Reports
\newcommand\physscr{{Phys.~Scr}}   % Physica Scripta
\newcommand\planss{{Planet.~Space~Sci.}}   % Planetary Space Science
\newcommand\procspie{{Proc.~SPIE}}   % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
